Action Genome: Actions as Composition of Spatio-temporal Scene Graphs

Action recognition has typically treated actions and activities as monolithic events that occur in videos. However, there is evidence from Cognitive Science and Neuroscience that people actively encode activities into consistent hierarchical part structures. However in Computer Vision, few explorations on representations encoding event partonomies have been made. Inspired by evidence that the prototypical unit of an event is an action-object interaction, we introduce Action Genome, a representation that decomposes actions into spatio-temporal scene graphs. Action Genome captures changes between objects and their pairwise relationships while an action occurs. It contains 10K videos with 0.4M objects and 1.7M visual relationships annotated. With Action Genome, we extend an existing action recognition model by incorporating scene graphs as spatio-temporal feature banks to achieve better performance on the Charades dataset. Next, by decomposing and learning the temporal changes in visual relationships that result in an action, we demonstrate the utility of a hierarchical event decomposition by enabling few-shot action recognition, achieving 42.7% mAP using as few as 10 examples. Finally, we benchmark existing scene graph models on the new task of spatio-temporal scene graph prediction.

==> figures/fig-bipartite.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/bipartite.pdf}
    \caption{(a) A weighted bipartite mapping between the objects to the relationships. The weights represent how the percentage of all relationships occurrences in which the specific object and relationship occur together. There are three colors in the graph and they represent the three kinds of relationships: attention, spatial and semantic. We find that (b) semantic, (c) attention, and (d) spatial relationships are involved with a wide variety of objects. (e) While most objects like ``door'' are involved in a variety of relationships, (f) a few objects and relationships are only involved in 1 or 2 relationships and objects, respectively.}
    \label{fig:bipartite}
\end{figure*}

==> tables/tab-sgg-benchmark.tex <==
\begin{table*}[]
\centering
\caption{We evaluate numerous recently proposed image-based scene graph prediction models and provide a benchmark for the new task of spatio-temporal scene graph prediction. We find that there is significant room for improvement, especially since these existing methods were  designed to be conditioned on a single frame and do not consider the entire video sequence as a whole.}
\begin{tabular}{@{\extracolsep{4pt}}llllllllll@{}}
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{3}{c}{\texttt{PredCls}} & \multicolumn{3}{c}{\texttt{SGCls}} & \multicolumn{3}{c}{\texttt{SGGen}} \\ \cline{2-4}\cline{5-7}\cline{8-10} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c}{R@50} & \multicolumn{1}{c}{R@100} & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c}{R@50} & \multicolumn{1}{c}{R@100} & \multicolumn{1}{c}{R@20} & \multicolumn{1}{c}{R@50} & \multicolumn{1}{c}{R@100} \\ \hline \hline
\texttt{VRD}~\cite{lu2016visual} & 24.92 & 25.20 & 25.22 & 22.59 & 24.62 & 25.08 & 16.40 & 17.27 & 17.37 \\
\texttt{Freq Prior}~\cite{zellers2017neural} & 45.50 & 45.67 & 45.67 & 43.89 & 45.60 & 45.67 & 33.37 & 34.54 & 34.60 \\ 
\texttt{Graph R-CNN}~\cite{yang2018graph} & 23.71 & 23.91 & 23.92 & 21.76 & 23.50 & 23.83 & 15.99 & 16.81 & 16.90 \\
\texttt{MSDN}~\cite{li2017scene} & 48.05 & 48.32 & 48.33 & 44.69 & 47.85 & 48.26 & 34.18 & 36.09 & 36.29 \\
\texttt{IMP}~\cite{xu2017scene} & 48.20 & 48.48 & 48.49 & 44.78 & 48.00 & 48.42 & 34.24 & 36.18 & 36.39 \\ 
\texttt{RelDN}~\cite{zhang2019graphical} & \textbf{49.37} & \textbf{49.58} & \textbf{49.58} & \textbf{46.74} & \textbf{49.36} & \textbf{49.57} & \textbf{35.61} & \textbf{37.21} & \textbf{37.33}
\end{tabular}
\label{tab:benchmark}
\end{table*}
